A thermo-mechanical phase-field fracture model: application to hot cracking simulations in additive manufacturing

Thermal fracture is prevalent in many engineering problems and is one of the most devastating defects in metal additive manufacturing. Due to the interactive underlying physics involved, the computational simulation of such a process is challenging. In this work, we propose a thermo-mechanical phase-field fracture model, which is based on a thermodynamically consistent derivation. The influence of different coupling terms such as damage-informed thermomechanics and heat conduction and temperature-dependent fracture properties, as well as different phase-field fracture formulations, are discussed. Finally, the model is implemented in the finite element method and applied to simulate the hot cracking in additive manufacturing. Thereby not only the thermal strain but also the solidification shrinkage are considered. As for thermal history, various predicted thermal profiles, including analytical solution and numerical thermal temperature profile around the melting pool, are regarded, whereas the latter includes the influence of different process parameters. The studies reveal that the solidification shrinkage strain takes a dominant role in the formation of the circumferential crack, while the temperature gradient is mostly responsible for the central crack. Process parameter study demonstrates further that a higher laser power and slower scanning speed are favorable for keyhole mode hot cracking while a lower laser power and quicker scanning speed tend to form the conduction mode cracking. The numerical predictions of the hot cracking patterns are in good agreement with similar experimental observations, showing the capability of the model for further studies.

==> draft.tex <==
% why showing this?
%As for the standard linear theory of elasticity for isotropic solids, the elastic strain energy is given by
%\begin{equation}\label{eq:31}
%    \Psi_e =\int_\Omega \psi_e(\pmb{\varepsilon}_e,d) d\Omega
%\end{equation}

%, $\otimes$ is the outer product operation on the Eigen vectors.

The damaged elastic free energy density $\psi_e^{+}$ is expressed as a function of the principal strains, in which

\begin{equation}
    \int_\Gamma G_c(T) dA=\int_\Omega G_c(T) \gamma (d, \nabla d) dV,
\end{equation}

\begin{equation}\label{eq:57}
    \rho \dfrac{\partial \psi}{\partial \pmb\varepsilon}=\pmb\sigma, \quad \rho\dfrac{\partial\psi}{\partial d}=K, \quad \rho \dfrac{\partial \psi}{\partial(\nabla d)}=H, \quad \dfrac{\partial \psi}{\partial T}=\eta,
\end{equation}

%\textcolor{red}{Further, the model was combined with the phenomenological PBF model [3] to investigate hot cracking. The results are well coherent with previous numerical and experimental findings, demonstrating the proposed model is capable of capturing the crack patterns in thermal shock problems and the PBF process.}
%\textcolor{purple}{do not use abbreviation in the abstract... also no references as much as possible... stick to one tense usually present tense is preferred.}

 %\textcolor{purple}{please complete this part by reviewing some fundamental papers on the numerical and experimental side of the thermal fracture... See \cite{Liu2015} ...}  
 
 % GENERAL remarks\\
% - avoid black spaces as much as u can by moving the text a bit \\
% -for figs and eqs do not use (), and put space between Fig and its number.\\
% - try to make the figs size to be aligned with the margin text. for many figs u can make them bigger or arrange them in a way to do that. \\
% - please make the margin bigger. \\
% - the figures for the results section are not consistent at all! all should have the same size and much better quality/resolution. \\
% - please check every new paragraph u write with grammerly \\
% - put dot at the end of fig captions.

%\textcolor{purple}{nice start, simply add 5-10 relevant works where people look at the cracking in AM.}
% Due to the drawbacks of re-meshing to simulate cracks using the finite element method, the extended finite element (XFEM) has been adopted to investigate crack mechanisms
% \textcolor{purple}{re-meshing has nothing to do with or against XFEM, it is always an option... why liu2019novel}

% \textcolor{purple}{we need more RECENT works as well many of the above ones are good but old!... 
% \cite{FELDER2022103142}
% \cite{JIANG2020106713}
% \cite{Sarkar2020}
% }

% \textcolor{purple}{cite some review papers regarding application and numerics: Wu and de Lorenzis}.

% \textcolor{purple}{work of Wu group is completely missed! at least add 2 of them... nothing on CPF? ... also weissmann works?}

% \textcolor{purple}{you need a pic for the continuum potato and showing different fields and BCs schematically.... $\Omega$ and $\partial\Omega$ represent a spatial region and its boundary.}

% \textcolor{purple}{what about other variables and quantities? all have to be defined.}

% WHERE DID YOU GET THIS? ... To develop a thermodynamically consistent model, the Helmholtz free energy $\psi$ should be a convex function with respect to each variable. 

% \textcolor{purple}{you still did not defined $k$ the following points should be integrate in other ways through out the following definition not here!\\
% Note that in this work we assume that: 
% 1. the thermal conductivity $k$ degrades as a result of damage evolution
% 2. the fracture toughness $G_c$ is temperature-dependent.
% }

% WHY WE NEED THIS??
%Thus applying the chain rule
%\begin{equation}\label{eq:23}
%    \dot{\psi}=\dfrac{\partial \psi}{\partial \boldsymbol\varepsilon}: \dot{\boldsymbol\varepsilon}+\dfrac{\partial \psi}{\partial d} \dot{d}+\dfrac{\partial \psi}{\partial(\nabla d)} \cdot \nabla \dot{d}+\dfrac{\partial \psi}{\partial T}\dot{T}
%\end{equation}


%Despite the previous models, how to treat the length scale i.e. as material property or pure numerical parameter, and correspondingly the choice of the degradation function is still an open question.

% \textcolor{purple}{summarize it in a table form... also you can repeat the expressions for sigma, Y and ect. (const. relations).. also get rid of $c_0$ and put is as $\pi$?}

% In this work, the thermal energy is given by \textcolor{purple}{(Clayton, 2005)???}
% \begin{equation}
%     \Psi_T=\int_{\Omega}\rho \psi_T d\Omega=-\int_{\Omega}\rho c T~\text{log}(\dfrac{T}{T_0})d\Omega.
% \end{equation}
% Note that the dissipating heating effects due to fracture are not considered, i.e., damage increase does not provide a heat source.

and shows schematically in Fig. \ref{fig:Fig_1_motivation}.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{plot/thermo_mech_coupled_fracture.jpg}
%     \caption{thermomechanical coupled fracture}
%     \label{fig:thermo_mech_coupled_fracture}
% \end{figure}
%  \begin{table}[H]
%       \centering
%       \caption{CPF model for themo-elastic fracture}
%         \begin{center}
%         \begin{tabular}{c c c c c c c c} 
%         \hline
%         & Displacement sub-problem & Damage sub-problem & Thermal sub-problem 
%         \hline
%         Governing equations    & $\nabla \cdot \boldsymbol\sigma=0 $    & $\dfrac{G_{c}}{c_0\ell_{0}} \omega'(d)-\dfrac{2 G_{c}\ell_{0}}{c_0} \nabla^{2} d- Y=0 $
%         &  $k\nabla^2T=\rho c \dot T\-T(\dfrac{\partial \boldsymbol \sigma}{\partial T}:\dot{\boldsymbol\varepsilon}+\dfrac{\partial K}{\partial T } \dot d+\dfrac{\partial H}{\partial T } \nabla \dot d)-Q $\\
%         \hline
%         Constitutive relations & $\boldsymbol \sigma = \omega (d) \mathbb{C}^{e} (\boldsymbol \varepsilon - \boldsymbol \varepsilon_T) $ &
%         $-Y = \ome '(d) \max _{t} \psi_e^{+}(\boldsymbol\varepsilon_e,t)$  &
%         $\boldsymbol q = - k \nabla T$ \\
%         Boundary cnditions    & $\boldsymbol \sigma\cdot \boldsymbol{n}=\boldsymbol{t}^{\ast}$  & $\nabla d\cdot \boldsymbol{n}=0$  &
%         $\boldsymbol{q}\cdot \boldsymbol{n}=\boldsymbol{q}^{\ast}$        \\
%         Initial conditions & $\boldsymbol{u}(\boldsymbol{x}, 0)=\mathbf0 $ & 
%         $d(\boldsymbol{x}, 0) =0 $ &
%         $T(\boldsymbol{x}, 0)={T}_0(\boldsymbol{x}) $\\
%         \hline
%         \end{tabular}
%         \end{center}
%         \label{tab:thermal PFmodel}
% \end{table}

% \textcolor{purple}{be consistent and use "boldsymbol" everywhere instead of "boldsymbol"!}
%   $\delta_F \in \mathscr{V}_{F}$  ,

%Note that integration by parts and has been carried out where appropriate. Neumann boundary conditions have been used in the derivation of Eq. (72) and Dirichlet boundary conditions are introduced in the choice for spaces $\mathscr{U}_F$.

%where ($\cdot, \cdot$ ) denotes the inner product of functions.

%Specifically, we define the following spaces for all test and trial functions
%\begin{equation}
%\begin{array}{ll}
%\begin{aligned} 
%\mathscr{U}_{u} &:=\left\{\boldsymbol u \mid \boldsymbol u(x)=\boldsymbol u^{*}, \forall \boldsymbol x \in \partial \Omega_{u}\right\}, & 
%\mathscr{V}_{u} &:=\left\{{\psi}_{u} \mid {\psi}_{u}(\boldsymbol{x})=\boldsymbol{0}, \forall \boldsymbol{x} \in \partial \Omega_{u}\right\}, \\ 

%\mathscr{U}_{d} &:=\{d \mid d(\boldsymbol{x}) \in[0,1], \dot{d}(\boldsymbol{x}) \geq 0, \forall \boldsymbol{x} \in \Gamma\}, &
%\mathscr{V}_{d} &:=\{\psi_{d}\mid \psi_{d}(\boldsymbol{x}) \geq 0, \forall \boldsymbol{x} \in \Gamma\}, \\

%\mathscr{U}_{T} &:=\left\{T \mid T(\boldsymbol{x})=T^{*}, \forall \boldsymbol{x} \in \partial \Omega_{T}\right\}, & 
%\mathscr{V}_{T} &:=\left\{\psi_{T} \mid \psi_{T}(\boldsymbol{x})=0, \forall \boldsymbol{x} \in %\partial \Omega_{T}\right\} 
%\end{aligned}
%\end{array}
%\end{equation}

% In the finite element formulation, the set of unknowns can be formulated in a vector form as $\boldsymbol x$ , and consequently, the corresponding residual vector $\boldsymbol r$ takes a vector form defined as
% \begin{equation}
%     \boldsymbol{x}=[{x}_{u} \quad {x}_{d} \quad {x}_{T} ]\quad
% \boldsymbol{r}=[\boldsymbol r_{u} \quad \boldsymbol r_{d} \quad \boldsymbol r_{T} ]
% \end{equation}
% The discrete non-linear system is solved by the Newton-Raphson method at every time step. The nonlinear residual at a time step can be written as $\boldsymbol r = \boldsymbol r(\boldsymbol x) = 0$ . The solution of the problem at the $(k + 1)^{th}$ Newton iteration is $\boldsymbol x_{k +1} = \boldsymbol x_k + \Delta \boldsymbol x_k$, where $\Delta \boldsymbol x_k$ is the solution of the update equation
% \begin{equation}
%     \boldsymbol K\left(\boldsymbol x_{k}\right) \Delta \boldsymbol x_{k}=-\boldsymbol r\left(\boldsymbol x_{k}\right)
% \end{equation}
% The stiffness matrix of the finite element formulation of this model takes the following block structure
% \begin{equation}
%     \boldsymbol{K}=\left[\begin{matrix}
% \boldsymbol{K}_{ u  u} & \boldsymbol{K}_{ u d} & \boldsymbol{K}_{ u T}  \\ 
% \boldsymbol{K}_{d  u} & \boldsymbol{K}_{d d} & \boldsymbol{K}_{d T}  \\ 
% \boldsymbol{K}_{T  u} & \boldsymbol{K}_{T d} & \boldsymbol{K}_{T T}  \\ 
%     \end{matrix}\right]
% \end{equation}
% where the first subscript of each block indicates which residual equation is differentiated and the second subscript indicates the variable it is being differentiated with respect to.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{plot/single_notch_mesh_tri.jpg}
%     \caption{Single edge notched tension test. (a) Geometry, dimensions and boundary conditions. (b) Unstructured mesh with refined mesh along the anticipated crack path.}
%     \label{fig:single_notche_tension}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.1\textwidth]{plot/non-fully coupled comparison.jpg}
%     \caption{Comparison of temperature field and crack propagation between non-coupled and fully-coupled case at 0.37us, 0.43us and 0.49us. 
%     \textcolor{red}{very small! :( why reporting time step? simply use time... i still do not understand why it is fully red for the lower right hand side... why u chose these timesteps? in all of them either there is no crack or suddenly fully cracked}}
%     \label{fig:comparison_non_fully}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{plot/Flux_com.jpg}
%     \caption{Snapshots of heat flux magnitude and direction of fully-coupled model and for non-coupled model at 0.39 ms.}
%     \label{fig:Flux_com}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{plot/k_flux.jpg}
%     \caption{comparison of thermal conductivity and heat flux of non-and fully-coupled case. 
%     \textcolor{red}{VERY SMALL! why!? make the margin bigger make the figure bigger, so many good info are all hidden and not visible at all!} }
%     \label{fig:T_Flux}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{plot/T_convergence.pdf}
%     \caption{Temperature field along cross section with different $\ell_{0}$.}
%     \label{fig:T_convergence}
% \end{figure} 
% Besides the insensitivity study of reaction force with respect to $\ell_{0}$, we also check the temperature profile's convergence of the CPF model. The temperature fields along line segment A-A at the same specific time t = 0.40 ms with different length-scale are plotted in Fig. \ref{fig:T_convergence}. The temperature of the whole specimen is lower than the initial temperature $T_0$. In the damaged region, the crack phase field increases as approaches the center, as Fig. \ref{fig:d_profile_wu_power} shows. Meanwhile, the temperature is decreasing from the top and bottom boundaries to the center, and in the center of the cracked region, the temperature achieves the minimum value, as a result of the "cooling down" effect. While in the intact regions the temperatures are almost equal with different $\ell_{0}$, which means the CPF model also holds convergence with different length-scale.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{plot/crack_T_changeT_k0.jpg}
%     \caption{Single edge notched tension test under mechanical and temperature loading and without thermal conductivity degradation. Crack pattern and temperature profile with decreasing temperature (left column), constant temperature (middle column) and increasing temperature (right column).}  
%     \label{fig:crack_T_changeT_k0}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.60\textwidth]{plot/T_final_chang_T.pdf}
%     \caption{Temperature field along line segment A-A with degraded thermal conductivity and constant thermal conductivity for the three cases.}  
%     \label{fig:T_final_chang_T}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{plot/quenching_mesh.jpg}
%     \caption{Geometry and boundary conditions for quenching test: (a) the whole specimen; (b) the model of a quarter of the whole specimen and (c) the mesh for the model.}
%     % \textcolor{red}{design each fig wisely! show the mesh as well! why empty space... show the full BVP and zoom in to the quarter for example.}
%     \label{fig:geometry for quenching test}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{plot/quenching_d_T.jpg}
%     \caption{Snapshots of quenching test with $T_0$ = 300 $^{\circ}$C and $T_a$ = 20 $^{\circ}$C at 10 ms, 50 ms and 200 ms: (a) crack evolution and (b) temperature field evolution.}
%     % \textcolor{red}{three row is enough why showing 4? omit the third row? I suggest u use different color bat for temp, it is exactly the same as damage and can be very confusing.}
%     \label{fig:temperature profile and crack evolution of quenching test}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\textwidth]{plot/quenching_experiment.png}
%     \caption{Comparison of crack pattern between numerical and experimental result \cite{jiang2012study}}
%     \label{fig:crack pattern comparison at 300}
% \end{figure}



% %%%
% \subsection{Thermo-mechanical coupled fracture}
% Many investigations focus on this aspect of fracture from the experimental side. Kokinl et al. \cite{kokini1997thermal} studied the thermal fracture mechanisms in ceramic thermal barrier coatings experimentally and analytically. Liu et al. \cite{Liu2015} conducted both thermal shock experiments with thin circular ceramic specimens and numerical simulations based on the minimum potential energy principle. For this thermo-mechanical coupled fracture problem, there are various other numerical methods developed through the years which can address the fracture problem in solids. For example, one can mention eXtended finite element methods (XFEM), boundary element method (BEM), or cohesive zone models (CZM). Interestingly enough, one can see the application of such models for thermo-mechanically coupled scenarios as well.

% Computational modeling of thermal fracture is studied extensively with different approaches. 
% Duflot et al. \cite{duflot2008extended} applied XFEM to the simulate thermally stressed cracked solids where both thermal and mechanical fields are enriched to represent the discontinuous
% temperature, heat flux, displacement, and traction across the crack surface.
% Jiang et al. \cite{JIANG2020106713} also utilized XFEM to study the thermo-mechanical fracture of ceramic nuclear fuel for both prescribed stationary cracks and propagating cracks in a multiphysics framework.
% Tarasovs et al. \cite{tarasovs2014self} predicted the crack pattern formation due to thermal shock loading at the surface of half-space using the two-dimensional BEM. See also work of Bahre et al. \cite{bahr1988multiple}.
% CZM is used to study the interface fracture under thermal-mechanical loading as well. See investigations by \cite{ozdemir2010thermo, hattiangadi2005numerical, FAGERSTROM20083037}. However, all the aforementioned discontinuous approaches to fracture require specific failure criteria and the discontinuous crack surface has to be explicitly tracked, making it difficult to solve arbitrary and complex crack problems.
% Continuum damage mechanics (CDM) based models are used to reproduce multiple cracking patterns of thermal shock. For example, Tang et al. \cite{tang2016numerical} developed a finite element model to simulate the thermal cracking behavior of heterogeneous brittle solids subjected to thermal shock. See also \cite{wang2013thermal, dube2010modeling} for similar studies. 
% Felder et al. \cite{FELDER2022103142} proposed a thermo-mechanical coupled gradient extended damage plasticity model for metallic materials to analyze ductile fracture and the corresponding thermal coupling effects. 
% Sarkar et al. \cite{Sarkar2020} proposed a thermo-mechanical formulation for conventional and localizing gradient damage methods, which are based on the generalized micromorphic theory and account for the underlying fracture process at the micro-level.

% Recently Peridynamics (PD), as a meshfree method is utilized to simulate the crack propagation and branching of materials  \cite{silling2000reformulation}.  It formulates the cracking behavior by estimating the summation of forces at each main particle exerted by the surrounding particles in terms of integral equations, so neither partial differential equations nor derivatives are needed. See the investigations in \cite{wang2018peridynamic, li2020thermally} for the application of PD in thermal fracture. However, one of the major challenges for PD is the treatment of boundary conditions in a non-local fashion \cite{diehl2019review}. The meshless discretization of PD is computational intensive similar to molecular dynamics, which may increase the computational efforts tremendously. 


% For example, one can mention eXtended finite element methods (XFEM), boundary element method (BEM), or cohesive zone models (CZM). However, all the aforementioned approches, the discontinuous crack surface has to be explicitly tracked, making it difficult to solve arbitrary and complex crack problems. Recently Peridynamics (PD), as a meshfree method is utilized to simulate the crack propagation and branching of materials \cite{silling2000reformulation}. However, one of the major challenges for PD is the treatment of boundary conditions in a non-local fashion \cite{diehl2019review}. The meshless discretization of PD is computational intensive similar to molecular dynamics, which may increase the computational efforts tremendously. 
